Maximizing Slice-Volumes of Semialgebraic Sets using Sum-of-Squares Programming

This paper presents an algorithm to maximize the volume of an affine slice through a given semialgebraic set. This slice-volume task is formulated as an infinite-dimensional linear program in continuous functions, inspired by prior work in volume computation of semialgebraic sets. A convergent sequence of upper-bounds to the maximal slice volume are computed using the moment-Sum-of-Squares hierarchy of semidefinite programs in increasing size. The computational complexity of this scheme can be reduced by utilizing topological structure (in dimensions 2, 3, 4, 8) and symmetry. This numerical convergence can be accelerated through the introduction of redundant Stokes-based constraints. Demonstrations of slice-volume calculation are performed on example sets.

==> sections_mp/abstract.tex <==
\abstract{


\urg{The destination of this paper will probably be 
% \href{https://mpc.zib.de/index.php\textbf}
% {Mathematical Programming Computation}.
Mathematical Programming Computation \texttt{https://mpc.zib.de/index.php\textbf}.

There's an issue in the Springer nature template w.r.t. referencing the Subequations environment. I'm not entirely sure what is occurring.
}

This paper presents an algorithm to maximize the volume of an affine slice through a given semi-algebraic set. This slice-volume task is formulated as an infinite-dimensional linear program in continuous functions, inspired by prior work in volume computation of semialgebraic sets. A convergent sequence of upper-bounds to the maximal slice volume are computed using the moment-Sum-of-Squares hierarchy of semidefinite programs in increasing size. The computational complexity of this scheme can be reduced by utilizing topological structure (in dimensions 2, 3, 4, 8) and symmetry.
This numerical convergence can be accelerated through the introduction of redundant Stokes-based constraints. Demonstrations of slice-volume calculation are performed on example sets.}
